Control Exchange Points: Providing QoS-enabled End-to-End Services via SDN-based Inter-domain Routing Orchestration

This paper presents the vision of the Control Exchange Point (CXP) architectural model. The model is motivated by the inflexibility and ossification of today's inter-domain routing system, which renders critical QoS-constrained end-to-end (e2e) network services difficult or simply impossible to provide. CXPs operate on slices of ISP networks and are built on basic Software Defined Networking (SDN) principles, such as the clean decoupling of the routing control plane from the data plane and the consequent logical centralization of control. The main goal of the architectural model is to provide e2e services with QoS constraints across domains. This is achieved through defining a new type of business relationship between ISPs, which advertise partial paths (so-called pathlets) with specific properties, and the orchestrating role of the CXPs, which dynamically stitch them together and provision e2e QoS. Revenue from value-added services flows from the clients of the CXP to the ISPs participating in the service. The novelty of the approach is the combination of SDN programmability and dynamic path stitching techniques for inter-domain routing, which extends the value proposition of SDN over multiple domains. We first describe the challenges related to e2e service provision with the current inter-domain routing and peering model, and then continue with the benefits of our approach. Subsequently, we describe the CXP model in detail and report on an initial feasibility analysis.

==> utils.tex <==
%%%
%%% Figure stuff
%%%
\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}
\renewcommand{\textfraction}{0}
%\renewcommand{\baselinestretch}{.985}

%%
%% General definitions one needs all the time
%%

\newcommand{\nibp}{\noindent\hspace{0.3em}\textbullet\hspace{0.7em}}

\newcommand{\xref}[1]{Section~\ref{#1}}
%\newcommand{\xref}[1]{\S\ref{#1}}
\newcommand{\cref}[1]{Chapter~\ref{#1}}
\newcommand{\pxref}[1]{(\xref{#1})}
\newcommand{\fref}[1]{Figure~\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\see}[1]{~(see \xref{#1})}
\newcommand{\first}{\emph{(i)}~}
\newcommand{\second}{\emph{(ii)}~}
\newcommand{\third}{\emph{(iii)}~}
\newcommand{\fourth}{\emph{(iv)}~}
\newcommand{\fifth}{\emph{(v)}~}
\newcommand{\sixth}{\emph{(iv)}~}

\newcommand{\zb}{z.\,B. \@}

\newcommand{\ie}{i.e., \@}
\newcommand{\eg}{e.g., \@}
\newcommand{\etc}{etc., \@}
\newcommand{\Ie}{That is, \@}
\newcommand{\Eg}{For example, \@}
\newcommand{\cf}{cf. \@}
\newcommand{\Cf}{Cf. \@}

\newcommand{\etal}{et~al.\xspace}

\newcommand{\perc}{\,\%\xspace}
\newcommand{\pert}{\,\textperthousand\xspace}

\newcommand{\checked}{\ding{52}\xspace}
\newcommand{\unchecked}{\ding{56}\xspace}

\newcommand{\lstfun}[1]{function \lstinline[basicstyle=\normalsize]{#1}\xspace}
\newcommand{\lstfuns}[2]{functions \lstinline[basicstyle=\normalsize]{#1} and \lstinline[basicstyle=\normalsize]{#2}\xspace}

% "smallitemize"-environment like "itemize" but more dense
\newenvironment{smallitemize}{%
\begin{itemize}%
\setlength{\parsep}{0.3ex}%
%\setlength{\itemindent}{-3ex}%
\setlength{\leftmargin}{0.1pt}%
\setlength{\listparindent}{-8ex}%
\setlength{\itemsep}{0.2ex}%
\setlength{\topsep}{0ex}%
\setlength{\parskip}{0ex}%
\setlength{\partopsep}{0ex}%
}{%
\end{itemize}
}%

% "smallenumerate"-environment like "enumerate" but more dense
\newenvironment{smallenumerate}{%
\begin{enumerate}%
\setlength{\parsep}{0.3ex}%
%\setlength{\itemindent}{-3ex}%
\setlength{\leftmargin}{0.1pt}%
\setlength{\listparindent}{-8ex}%
\setlength{\itemsep}{0.2ex}%
\setlength{\topsep}{0ex}%
\setlength{\parskip}{0ex}%
\setlength{\partopsep}{0ex}%
}{%
\end{enumerate}
}%

\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{brown}{rgb}{0.7,0.3,0}
\definecolor{darkblue}{rgb}{0,0,0.5}
\newcommand{\todo}[1]{\textit{\textcolor{red}{TODO: #1}}}
%\newcommand{\bernhard}[1]{\textit{Bernhard: #1}}
\newcommand{\vassilis}[1]{\textit{\textcolor{brown}{#1---Vassilis.}}}
\newcommand{\fontas}[1]{\textit{\textcolor{darkblue}{#1---Fontas.}}}
\newcommand{\bernhard}[1]{\textit{\textcolor{darkgreen}{#1---Bernhard.}}}

%\renewcommand{\todo}[1]{}

% mark changed wording from first submission
\newcommand{\new}[1]{\textcolor{blue}{#1}}
\newcommand{\discuss}[1]{\textit{\textcolor{green}{Discuss: #1}}}

%\definecolor{mygrey}{rgb}{0.8,0.8,0.8}

\newcounter{fn1}
\setcounter{fn1}{1}
\newcounter{fn2}
\setcounter{fn2}{2}
\newcounter{fn3}
\setcounter{fn3}{3}
\newcounter{fn4}
\setcounter{fn4}{4}
\newcounter{fn5}
\setcounter{fn5}{5}
\newcommand{\fnsym}[1]{$^{\fnsymbol{#1}}$}

\newcommand{\minisec}[1]{\noindent\textbf{#1}:}

%%%
%%% Definitions specific to some papers
%%%

\newcommand{\libpcap}{\textsc{libpcap}\xspace}
\newcommand{\winpcap}{\textsc{winpcap}\xspace}
\newcommand{\libz}{\textsc{libz}\xspace}
\newcommand{\tcpdump}{\textsc{tcpdump}\xspace}
\newcommand{\snort}{\textsc{snort}\xspace}
\newcommand{\ipsumdump}{\textsc{ipsumdump}\xspace}
\newcommand{\wireshark}{\textsc{Wireshark}\xspace}
\newcommand{\bro}{\textsc{Bro}\xspace}
\newcommand{\spbc}{\textsc{spbc}\xspace}


\newcommand{\centralization}{Routing Centralization\xspace}
\newcommand{\raas}{Routing-as-a-Service\xspace}

